Learning Attribute-Based and Relationship-Based Access Control Policies with Unknown Values

Attribute-Based Access Control (ABAC) and Relationship-based access control (ReBAC) provide a high level of expressiveness and flexibility that promote security and information sharing, by allowing policies to be expressed in terms of attributes of and chains of relationships between entities. Algorithms for learning ABAC and ReBAC policies from legacy access control information have the potential to significantly reduce the cost of migration to ABAC or ReBAC. This paper presents the first algorithms for mining ABAC and ReBAC policies from access control lists (ACLs) and incomplete information about entities, where the values of some attributes of some entities are unknown. We show that the core of this problem can be viewed as learning a concise three-valued logic formula from a set of labeled feature vectors containing unknowns, and we give the first algorithm (to the best of our knowledge) for that problem.

==> conclusion.tex <==
% !TeX root = main.tex

\section{Future Work}
\label{sec:conclusion}

%This paper presents a new ReBAC policy mining algorithms based on decision tree learning and an evaluation comparing our new algorithms with the state-of-the-art ReBAC policy mining algorithms: Iyer et al.'s mining authorization policies algorithm \cite{iyer2019} and FS-SEA* \cite{bui19sacmat}. Compared to Iyer et al.'s algorithm, our algorithms can mine syntactically better policies and are several times faster. Compared to FS-SEA*, DTRM is simpler, significantly faster, and achieves comparable policy quality. Mining ReBAC policies with negation is another significant contribution over the previous works.

Directions for future work include: extending our algorithms to handle incompleteness and noise in the ACLs, perhaps using decision tree pruning methods, which are designed to avoid overfitting; extending our algorithms to identify errors in attribute values, and possibly suggest corrections; 
%supporting additional policy language features, such as inheritance and transitive closure; 
and developing incremental algorithms that efficiently handle updates to the object model or authorizations.

%One is to augment our algorithm with an initial phase for feature selection, such as the feature selection phase in \cite{bui19sacmat}, and see whether this improves the policy quality, as it did for Bui et al.'s evolutionary algorithm.  
% extraneous permissions can be handled as we have done before with threshold to discard low quality rules, but missing permissions can't, I think.  tree pruning might handle them.

